COSMic: A Coherence-Aware Generation Metric for Image Descriptions

Developers of text generation models rely on automated evaluation metrics as a stand-in for slow and expensive manual evaluations. However, image captioning metrics have struggled to give accurate learned estimates of the semantic and pragmatic success of output text. We address this weakness by introducing the first discourse-aware learned generation metric for evaluating image descriptions. Our approach is inspired by computational theories of discourse for capturing information goals using coherence. We present a dataset of image$\unicode{x2013}$description pairs annotated with coherence relations. We then train a coherence-aware metric on a subset of the Conceptual Captions dataset and measure its effectiveness$\unicode{x2014}$its ability to predict human ratings of output captions$\unicode{x2014}$on a test set composed of out-of-domain images. We demonstrate a higher Kendall Correlation Coefficient for our proposed metric with the human judgments for the results of a number of state-of-the-art coherence-aware caption generation models when compared to several other metrics including recently proposed learned metrics such as BLEURT and BERTScore.

==> coco_results.tex <==
\begin{table*}[!hb]
    % \small
    \small
    \centering
    \begin{tabular}{p{1.5cm}p{3cm}p{3cm}p{3cm}p{3cm}}
         & \centering{\includegraphics[width=3cm,height=3cm]{img/coco_eval/img1.jpeg}} & 
         \centering{\includegraphics[width=3cm,height=3cm]{img/coco_eval/img2.jpeg}} & 
         \centering{\includegraphics[width=3cm,height=3cm]{img/coco_eval/img3.jpeg}} & 
         \includegraphics[width=3cm,height=3cm]{img/coco_eval/img4.jpeg} \\
         \textbf{Reference} & Windsurfing by the ocean shore & View of a building and city with a man to the side looking out onto the city & Holiday card featuring a cute reindeer at the North Pole & Two large skyscrapers with a rainbow light bridge running over a river between them at sunset \\
         \textbf{BUTD Generated} & a pink kite flying over a body of water & a large building with a large building in the background  & a picture of a dog that is on the ground & a view of a city and a city skyline \\
         \multirow{3}{*}{\textbf{COSMic}} & \center{0.413} & \center{0.841} & \center{0.446} & \center{0.899}\\
        %  \midrule
        %  & \includegraphics[width=3cm,height=3cm]{img/t2_comparison/img_5.jpg} & 
        %  \includegraphics[width=3cm,height=3cm]{img/t2_comparison/img_6.jpg} &
        %  \includegraphics[width=3cm,height=3cm]{img/t2_comparison/img_7.jpg} & 
        %  \includegraphics[width=3cm,height=3cm]{img/t2_comparison/img_8.jpg} \\
        %  \textbf{Reference} & mountains in front of a clear blue sky & person driving a blue motorcycle on a street & close-up of a bug hiding behind a blade of grass & white flowers on a bush \\
        %  \textbf{Generated Visible} & mountain range as seen from the trail & a view of a motorcycle & dragonfly on a blade of grass & white flowers on a bush \\
    \end{tabular}
    \caption{
        Illustration of the out-of-domain \t2cc reference captions and their generated captions using the Bottom-Up Top-Down COCO captioning model. Errors in the descriptions of the images lower the COSMic score, in the first and third images. Second and fourth images receive high scores because words in the generated captions match the ones in the reference and the image. Effect of the discrepancy between the image and the generated caption on the COSMic score is lower. Both the reference captions and the generated captions are in the Visible coherence class.
        See Table~\ref{tab:test_results} for average scores over the test set. (Photo credits, from left to right: \textcolor{red}{PUT PHOTO CREDITS HERE!!!!!!!!!!!!!!!})}
    \label{tab:butd}
\end{table*}

==> misc.tex <==
\begin{table} [!ht]
\small
\centering
\begin{tabular}{ccc}
\hline
    & \textbf{Number of Images} & \textbf{Percentage}\\
 \hline
 Meta & 265 & 86.6\%\\
 Visible &  243 & 79.4\%\\
 Action & 292 & 95.4\%\\
 Subjective & 219 & 71.6\%\\
 Story & 298 & 97.4\%\\
 Irrelevant & 297 & 97.1\%\\
 \hline
 Perfect Match & 109 & 35.6\% \\
 \hline
\end{tabular}

\caption{Number of images per category that the annotators agreed on. It is also counted when the annotators agreed that the same image is \textit{not} in the given category. Perfect match corresponds to when all the categories that were picked by an annotator for a single image matches all the categories picked by the other annotator.}
\label{tab:agreed_annotator_not}

\end{table}



\begin{table}[!ht]
\centering
\begin{tabular}{ccc}
\hline
    & \textbf{Number of Images} & \textbf{Percentage}\\
 \hline
 Meta & 258 & 84.3\%\\
 Visible &  25 & 8.17\%\\
 Action & 21 & 6.86\%\\
 Subjective & 66 & 21.57\%\\
 Story & 1 & 0.32\%\\
 Irrelevant & 4 & 1.31\%\\
 \hline
\end{tabular}
\caption{Number of images per category that the annotators agreed on. It is only counted when the annotators agree and that the same image is in the given category.}
\label{tab:agreed_annotator}
\end{table}

\begin{table}[!ht]
\small
\centering
\begin{tabular}{cp{0.4cm}p{0.6cm}p{0.6cm}p{0.5cm}p{0.5cm}p{0.4cm}}
\hline
 & \textbf{Meta} & \textbf{Visible} & \textbf{Action} & \textbf{Subj.} & \textbf{Story} & \textbf{Irr.} \\
 \hline
 Annotator 1 & 319 & 107 & 41 & 90 & 9 & 14\\
 Annotator 2 & 300 & 28 & 25 & 142 & 7 & 6 \\
\hline
\end{tabular}
\caption{Number of images per category that the annotators picked.}
\label{tab:annotator_kappa}
\end{table}


